Read Mapping Near Non-Volatile Memory

DNA sequencing is the physical/biochemical process of identifying the location of the four bases (Adenine, Guanine, Cytosine, Thymine) in a DNA strand. As semiconductor technology revolutionized computing, modern DNA sequencing technology (termed Next Generation Sequencing, NGS)revolutionized genomic research. As a result, modern NGS platforms can sequence hundreds of millions of short DNA fragments in parallel. The sequenced DNA fragments, representing the output of NGS platforms, are termed reads. Besides genomic variations, NGS imperfections induce noise in reads. Mapping each read to (the most similar portion of) a reference genome of the same species, i.e., read mapping, is a common critical first step in a diverse set of emerging bioinformatics applications. Mapping represents a search-heavy memory-intensive similarity matching problem, therefore, can greatly benefit from near-memory processing. Intuition suggests using fast associative search enabled by Ternary Content Addressable Memory (TCAM) by construction. However, the excessive energy consumption and lack of support for similarity matching (under NGS and genomic variation induced noise) renders direct application of TCAM infeasible, irrespective of volatility, where only non-volatile TCAM can accommodate the large memory footprint in an area-efficient way. This paper introduces GeNVoM, a scalable, energy-efficient and high-throughput solution. Instead of optimizing an algorithm developed for general-purpose computers or GPUs, GeNVoM rethinks the algorithm and non-volatile TCAM-based accelerator design together from the ground up. Thereby GeNVoM can improve the throughput by up to 113.5 times (3.6); the energy consumption, by up to 210.9 times (1.36), when compared to a GPU (accelerator) baseline, which represents one of the highest-throughput implementations known.

==> arch.tex <==
In this section, we explore different units of \arch\ introduced in Section~\ref{sec:biocam}
in more details. For each unit, we consider different sizes and designs (where applicable).
Then, all these design points are compared against each other in the Evaluation Section,
to find the most optimum \arch\ architecture.

\subsection{SSU}
This unit coordinates all accesses to databases containing sub-sequences and the final
matching indices. Since these sub-sequences are usually coming from an I/O source,
latency of communication can become a bottle-neck. So, SSU employs two simple queues (FIFOs)
to mask latency overheads. Considering different sizes for the queues, our analysis shows that
a queue of XXXKB for receiving the sub-sequences and a queue of YYYKB to write the final
indices back can effectively mask all such latency overheads.

\subsection{Filtering Unit}
As discussed in Section XXX, FU prunes the search space, considering part of the first bps
of the sub-sequence. To detail the architecture of this unit, we need to answer
two questions. First question is how many bps to use for filtering? To answer this question
we recall that a human genome contains around 3Gbps, so 3 billion locations. A 32-bit address
space is needed to point to each location uniquely. This is equivalent to 16bps. Since this
address space can cover a space larger than 3 billion locations, we consider 15 bps for
filtering unit as the maximum. A larger m prunes the search space significantly, with the
cost of a larger PMITIL and SGU overhead. On the other hand, a small m has negligible
PMITIL and SGU overhead, but a larger number of searches. 
To find the optimum number of bps for filtering in this trade-off space, we sweep it
in the range of 5, 10, and 15 and show the most optimum point (XXX these numbers may change
in the final version).

\input{mdevtbl}

Besides, we need to consider scenarios in which the first m bps of the sub-sequence
deviate from the reference. Then, in filtering mechanism, deviations from the exact m bps
should be searched as well. This is the role of SGU. Now, the second question is how many
bp deviation we should consider in the m bps? To answer this question, we recall that each
bp can deviate with 1\% chance. Considering this, if we do not explore any deviations
from the 15 bps (largest m explored), we cover
$$0.99^{15} \approx 86.0\%$$
on average, or equivalently, 13.9\% of the sub-sequences may not be aligned properly.
If we consider single bp deviation in the 15 bps, this time we can cover up to
$$0.99^{15} + {15 \choose 1} \times\ 0.01 \times 0.99^{14} \approx 99.0\%$$ on average.
So, having a SGU capable of searching for a single-bp deviated sub-sequence increase
the coverage by 13.0\% in comparison to a case that we do not include any SGU. Since
the coverage without SGU at all (86.0\%) is acceptable 
compared to the existing works [XXXX refs here], we explore both design options and compare the 
results in the evaluations section (Section XXX). Table~\ref{tbl:mdev} summarizes the coverage
rate based on the number of bp deviations considered in SGU (if at all). We see that in all cases
searching for single-bp deviation leaves less than 1\% of the sub-sequences uncovered by \arch.

Next, we assess the size of PMIT. This table keeps an entry per location of reference genome,
including the exact address in TCAM arrays. So, it has 3 Giga entries. As we discussed, 32-bit
addresses are needed to point to each of these 3 Giga locations. So, each entry is 4B long.
Totally, PMIT's size is around 12GB. We assume that this table (generated at a pre-processing
step) is located in the main memory, and the address to the first entry is passed
 to FU.

Finally, we explore different options for PMITIL table. As discussed before, this table 
has $4^m$ entries, each pointing to an address in PMIT and a number indicating the number
of entries that should be read from PMIT starting from the address. So, we need 
maximum of $2 \times 4B = 8B$
per entry of PMITIL table. 
%Based on different m values, Table~\ref{tbl:pmitil} summarizes
%the size of PMITIL table. As we see here, the size of this table can be in range of KB, or 
%as large as GB. 
If m is as small as 5, size of PMITIL table is $$4^5 \times 8 = 8KB$$. However, for a large m
like 15, the table can be as large as $$4^15 \times 8 = 8GB$$.
In the evaluation, for smaller sizes we assume a local memory bank (in the order of KBs) inside FU
keeps this information. When size of this table gets larger (order of MBs), we assume that
it is located in the main memory besides PMIT. In this case, an address pointing to the first
entry of PMITIL table is passed to the FU.

\subsection{TCAM Banks Unit}
We build \arch TCAM banks on top of existing designs such as [XXXengin1,2] with slight
modifications. As discussed in Section XXX, we need to shift the sub-sequence to search
it against a specific location in reference genome. So, Shifting Logic Unit (SLU) shifts
the sub-sequence to the row specified by information from PMIT, before feeding it to the 
Query Register of the array. Besides, instead of searching the whole array, we only search 
for the sub-sequence in the given row by PMIT information. So, per each search query
from FU, sub-sequence is shifted and corresponding row is activated. Then, 
the modified sense amplifier (as explained in Section XXX)
detects similarity. Since each row has a unique sense amplifier, A MUX chooses the output
of the specified row's sense amplifier, as the final {\em Match Signal}. On a {\em Partial
Match} scenario, if the first part of the sub-sequence matches, a second search operation
will compare the rest of sub-sequence to detect the match. After the search step(s),
if a match is indicated by the {\em Match Signal}, the location of this match is sent to
the SSU to be stored in the output database. To summarize, \arch employs the existing TCAM
array structure with 3 modifications; (i) a shifting unit to shift the sub-sequences (SLU),
(ii) a MUX to read per-row sense amplifiers, and (iii) a different $V_{ref}$ for the sense
amplifiers (explained in Section XXX) to detect similarity, rather than exact match only.

The other unit of TBU is Request Dispatching Unit (DPU). The primary goal of this unit
is to get the search requests from FU and forwards them to the right TCAM Bank.
This unit can play an important role in the performance of \arch. It is important to make
sure that search requests are distibuted evenly among different banks, to avoid overloading
a single bank with requests. We exploit different techniques to address this issue. 
In the first technique, 
while generating PMIT in the pre-processing step, we make sure that indices in the same
group are shuffled to make sure that potential accesses to the same bank do not stay
close in PMIT. This is discussed in more details in Section XXX (setup XXX). 
In the second technique, a buffer is attached to each TCAM Bank to make sure that RDU
does not stall due to having multiple accesses to the same bank. Our final technique is
to add a buffer to the RDU, in order to forward next requests in case one bank is not free.
Adding large buffers to TCAM Banks has high overhead as we have large number of banks
in \arch. However, it makes the RDU buffer smaller and simpler. We explore different options
for the sizes of TCAM Bank and RDU buffers to find the most optimum design.

\subsection{System Level Integration}

**** we need to think about it. But probably, user just specifies range of addresses to 
the accelerator, and takes care of the rest.

\subsection{Data Encoding} Genome is a sequence of 4 different types of base pairs
(bp). It is usually stored in fasta and fastq formats, by their
ASCII codes. TCAM arrays operate the search at bit granularity. In other words,
the sense amplifier uses the number of mismatching bits to
find similar sub-sequences. We prefer to translate the number 
of mismatches between the sequences to number of bit
mismatches. However, this entirely depends on the 
encoding used for different bps. Besides, in finding the similarity,
mismatches between different types of bps are identical to
us. So, any mismatch between the sequences should lead to
the very same number of bit mismatches. Hence, encoding
of the sequences becomes important.

Since it is not possible to get same number of bit mismatches when
bps are encoded using 2 bits, we encode each base pair using 3 bits.
We show that it is possible to find 4 different 3-bit long numbers
to represent the bps, each two having exactly 2-bit difference.
As an example, 111, 100, 010, and 001 can be used for encoding.
So, in this study, we stick to having a 3-bit encoding. Besides,
on any bp mismatch, exactly two bits would mismatch. This makes the design of
sense amplifier easier since we do not care about single mismatches
any more.

[[This paragraph may be eliminated. too much noise in evaluation!]]
We use two methods for encoding. The first method aims 
to keep the number of bit differences on a mismatch 
the same for mismatches between any two bps. 
This needs minimum of 3 bits to represent each base pair.
On a mismatch between two bps, exactly two
bits will be different. This scheme helps in designing a more
robust and reliable sense amplifier, since the similarity is 
defined more precisely. However, this scheme comes with area
penalty as we only needed 2 bits to store four different bp
types. In the second method, we use only two bits
to encode the bps. Using this scheme, we may have 1 or 2
bits different on a mismatch. So, designing the sense am-
plifier become more challenging, and it may generate more
number of false positives. Hence, a longer post processing
step is needed. We quantify the trade-off space of using these
two encoding schemes in Section XXX.

\subsection{Sensing Similarity}
We know that different genomes are not exactly the same,
although they are %more than 99\% 
similar. 
%Differences between two genomes come from polymorphism rate 
%(the natural differences in genomes) and the errors in measurements
%[XXX lecture]. 
Hence, in designing an alignment accelerator, 
we are looking for Similarity between a sub-sequence
and the reference genome, rather than an exact match. Currently in TCAM arrays, 
sense amplifiers are designed to detect the exact match. 
So, even a single bit mismatch leads to
triggering a mismatch signal for that row. We need to change
the 
%design of sense amplifier 
sensing mechanism in a way that {\em similarity} can be captured, as well as a {\em match}.

First, we take a look at how match detection is performed
in TCAMs. On a match (mismatch), each cell connects
an $R_{high}$ ($R_{low}$) to the Match Line (ML). For instance, in an array with row
size of 100 bits, on an exact match, 100 $R_{high}$s are connected
to the ML. However, if 90\% of the cells are matching the
query, 90 $R_{high}$s and 10 $R_{low}$s are connected to the
ML. This will lead to a different effective resistance, lower
in comparison to the exact match case. Since TCAMs are
designed to find exact matches, sense amplifiers are tuned to
%should be
%accurate enough to 
sense the difference between an exact
match and a case that only a single bit mismatches, which
means only a single $R_{low}$ is connected to the ML. 

To capture similarity rather than match-only, sense amplifier 
should be adjusted accordingly to accept a lower effective resistance
as a match. For instance, it can be set to triger a match signal when
less than 5 bits are mis-matching, which means having less than 5 $R_low$s
connected to the ML. This way, be changing the matching threshold of sense
amplifiers, TCAM arrays are capable of capturing similarity when difference
is small enough.

[[{\bf we may include UCSD comparison here}]]

As shown in Figure [XXX resistance gaps, like what shown in oral defense and Engin's],
the gap between effective resistance levels under different number of mismatching bits
decreases as number of mismatching bits grows. 
Besides, due to process variation and other sources of noise,
TCAM cells' resistance deviates from being exaxctly $R_{high}$ or $R_{low}$.
Hence, adjusting the sensing mechanism becomes more challenging as we try
to move the accepted threshold to lower effective resistance regions.
For instance let us assume that up to 3 bp difference is acceptable.
This means 6 $R_{low}$s are considered as a match, while having 8 and more $R_{low}$s
connected to the ML is not a match anymore. Then, due to process variation, there
might be scenarios that resistance levels of a row containing 6 $R_{low}$s become
less than a row with 8 ${R_{high}}$s, which will lead to a failure in sensing.

Since similarity is a fuzzy concept unlike exact-match, such inaccurarcies (if not negligible)
can be tolerated by definition. Specefically in sequence alignment applications,
a single strict expected similarity threshold does not exist. So, fualts of sensing
similarity (if small) can be tolerated by these applications. 
These inaccuracies can cause negligible levels of uncertainty, rather than
leading to produce unacceptable or wrong results.
In Section XXX, we
quantify these sensing inaccuracies for different similarity thresholds and array sizes.

 

[[XXX we may want to eliminate rest of this section]]

This is
why small $\frac{R_{high}}{R_{low}}$ ratio makes the design of sense 
amplifier much more challenging (XXX cite Engin). Besides, as the size of 
array and consequently the rows increase, sensing margin 
becomes smaller, leading to more challenging sense amplifier
design. Moreover, the other challenge in designing a sense
amplifier is that $R_{high}$ and $R_{low}$ are prone to process 
variation. So, the final effective resistance connected to the sense
line, $R_{eff}$, varies from the expected value. As shown in [cite
Hassan UCI], process variation alone can lead to scenarios
that sense amplifier fails to detect a match or a mismatch.
This variation should be considered in designing the sense
amplifier too.

Similarity is a fuzzy concept by definition, rather than a
simple match or mismatch. Acceptability of a similarity
level between two sequences depends on the application. In
genome alignment problem, we are looking for similar 
sequences, rather than exactly identical ones. So, sense 
amplifier can tolerate noise. In other words, considering process
variation and other limits, we can design a sense amplifier
that captures a match when we have more than a specific
number of bits (let say 90 bits) matching the query;
however, due to the effect of noise, sense amplifier may 
trigger a match signal on lower number of matching bits (like
80) as well. This fuzziness is acceptable, as long as we make
sure that all sequences with more than a specific number of
bits matching will trigger a match signal. We call this safe
threshold $R_{match}$, and we report it in percents. For instance,
a sense amplifier designed for $R_{match}$ = 75\% and row size of
128 bits, triggers match signal always when more than 96
bits are matching the query, while sometimes it may trigger
a false match signal when we have less than 96 bits matching. 
So, it can trigger false positives, but false negatives are
not acceptable. False positives are not catastrophic failures.
They are rather less similar matches. 
%We show in SectionXXX how
%many False Positives are generated and how different they are.
In section XXX, for different array sizes and
PVT conditions, we quantify the rate of false positives and
consequently, the acceptability of sense amplifier for this application. 
Besides, we show how different the false positives can get from the
expected threshold.

[[XXX we may want to eliminate this pragraph completely]]
Similarity rate between a sub-sequence and the reference
genome is always low, except where it aligns, which is very
rare. In alignment applications, we are looking for more than
95\% of the bps matching the reference. We use this  
in designing the sense amplifier to decrease the number of
false positives. Basically, we set the goal of designing the
sense amplifier to capture all the cases with similarity above
$R_{match}$. At the same time, we try to decrease the probability 
of generating a false positive for cases with low similarity. 





==> back.tex <==
1.Sequence Alignment Primer

- Alignment fidelity?

- Accuracy?

- Cartoon?

2.TCAM primer


%-------------------------------------------------------------------------------%
%-------------------------------------------------------------------------------%

\ignore{
\redHL{Barracuda + other acceleration attempts}
}

%-------------------------------------------------------------------------------%
%-------------------------------------------------------------------------------%

\noindent {\em Problem Statement:}
For two characters x and y (representing bases) from the nucleotide alphabet
$\sum\{A,C,G,T\}$,...
Alignment between the query $query=[1...n]$ and $reference=[1...l]$...
These schemes first generate an alignment matrix, which keeps the scores. Once
the matrix is computed, it should be processed to extract the best alignment. In
\arch\ all of these steps are taken care of in one step by the TCAM access.
In a sense, the scoring is hard-coded in similarity.

On errors: Each SA accelerator accepts an error threshold, e.g. allowing 10\%
error in sequencing 100bp reads allows for up to 10 incorrect base (mis)matches.
Termed "identification percentage"




==> biocam.tex <==
Sequence Alignment algorithms try to locate the best-matching parts of a very long
reference genome to given short sub-sequences. So, a database of short sub-sequences is fed
to such an algorithm as the input, along with a reference genome. 
In return, for each sub-sequence, 
it finds the indices that a high-similarity
match with the reference genome is detected. 
So, this process includes large number of searches.

\begin{figure*}[tp]
  %\vshrink{-0.4}
  \begin{center}
%\hspace{-0.62cm}
  \includegraphics[width=\textwidth]{FIG/system.pdf}
%\vshrink{0.2}
  \caption{Overview of BioCAM accelerator.
  \label{fig:biocam}}
\end{center}
%\vshrink{0.6}
\end{figure*}

We propose BioCAM, an in-memory accelerator, for sequence alignment. 
BioCAM performs search operations using modified TCAM arrays, which can find
matches energy efficiently.  Reference genome is stored in TCAM arrays while
sub-sequences are searched against different arrays. As shown in Figure 1,
BioCAM has three major units. Sub-sequence Service Unit (SSU) handles all communications to
the Database of Sub-sequences. It reads the sub-sequences from the database and writes back
the indices at which, 
a high-similarity match to the reference genome exists (output of application). 
Index Filtering Unit
(IFU) filters the potential locations a match may exist, based on base-pair patterns observed
in the sub-sequences. In other words, instead of looking for a
match in all possible indices of the reference genome, IFU helps to reduce the number of
locations to search for a match in. Finally, TCAM Bank Unit (TBU) holds the reference genome in
modified TCAM arrays. TCAMs are changed to be able to search for high-similarity matches,
rather than just an exact match. In the next sections, we explain each unit in more details.

\subsection{Sub-sequence Service Unit (SSU)}
%This unit has two roles (Figure 2). First, to read the sub-sequences from the database. Second,
%to write match index information back. For both reads and writes, a small memory (in the range
%of KBs) is embedded to mask database communication latencies. These small memories (SMU
%and MIIT) service to requests like a queue, employing two counters. Read Index Register (RIR)
%points to where a new read request should access, while Write Index Register (WIR) points to
%an already-read entry that can be written in the next write request. So, after each read or write
%request, these registers are incremented by one. Besides, before increasing RIR (WIR), SSCU
%checks that new RIR (WIR) should always be smaller than current WIR (RIR). SSU includes to
%registers, SSR and MIIR, to service the requests coming from other units of BioCAM.

%{\bf alternative explanation:} 
SSU orchestrates all communications to databases. It reads
sub-sequences from a database to be searched, and writes the match indices back.
Two small queues (4 KBs) are employed to mask latencies of communication. 

%\begin{figure}
  %\vshrink{-0.4}
%  \begin{center}
%\hspace{-0.62cm}
%  \includegraphics[width=\columnwidth]{FIG/SSU.pdf}
%\vshrink{0.2}
%  \caption{Overview of SSU.
%  \label{fig:ssu}}
%\end{center}
%\vshrink{0.6}
%\end{figure}

\subsection{Index Filtering Unit (IFU)}
Figure 3 depicts different units of IFU. As explained before, IFU filters the potential indices to
search for in reference genome. 
To do this, first m base-pairs (bps) of the sub-sequence stored in SSR
is used for filtering. 
IFU tries to point to potential matching indices based on first m bps of SSR.
Thus, a pre-processing step traverses over the reference genome, looking at different m-
bp combinations. For each one, the index of combination in reference genome is stored in
Potential Matching Indices Table (PMIT). Basically, after pre-processing step, PMIT includes the
exact places to search for a sub-sequence starting with any given m bps. This information 
includes the bank, column, and row in which those m bps are observed. So, it
helps in searching for a match in a very specific location, instead of blindly searching all banks, rows, and columns. 
Since a m-bp combination may appear in multiple indices of reference
genome, most of the time PMIT has many more than one entry for each m-bp combination.
Hence, a smaller table, PMIT Index Locator (PMITIL) which has $4^m$ entries, keeps the range of
addresses in PMIT corresponding to a specific m-bp combination. Basically, each entry of PMITIL
(out of $4^m$ ) corresponding to a unique m-bp combination, keeps the start and end indices 
in PMIT.

{\bf [Pipelining options here???]}

\begin{figure}
  %\vshrink{-0.4}
  \begin{center}
%\hspace{-0.62cm}
  \includegraphics[width=\columnwidth]{FIG/FU.pdf}
%\vshrink{0.2}
  \caption{Overview of IFU.
  \label{fig:ifu}}
\end{center}
%\vshrink{0.6}
\end{figure}

Besides, since we are looking for high-similarity match rather than exact match, for each m-bp,
similar m-bp sequences should be searched for as well. SGU’s role is to find out indices of all similar
m-bp sequences in PMITIL. 
%To do this, we have two option. 
Hence, SGU sequentially generates all
possible deviations from a given m-bp sequence, by changing base pairs one at a time to all
3 other possible base pairs. For instance, if $i^{th}$ base pair is C, SGU generates 3 
different m-bp sequences, replacing only the $i^{th}$ base pair with A, G, and T in each. 
We will show later in SectionXXX that changing one base-pair at a time to generate similar
sub-sequences covers above 99\% of the potential scenarios.

%The other one is to implement SGU as a TCAM
%as well (considering an array design which can capture similarities as well). Then, in a single
%cycle, searching the whole TCAM, all possible similar m-bp sequences are located. 

%We compare
%both options to find the most energy efficient design

\subsection{TCAM Banks Unit (TBU)}
This unit handles all search operations. It has two main parts. A Request Dispatching Unit (RDU)
gets the search request from IFU along with coordinates for the search. Then, it sends it to the
corresponding TCAM bank to search for it. After search operation is done and potential match
index is sent back to RDU, it forwards the information to SSU.

{\bf [Different scheduling policies for RDU XXX]}

The other unit is TCAM banks. Each banks stores part of the reference genome. Per request, it
searches for a given subsequence in the coordinates provided from IFU. Next section explains TCAM
Banks in more detail.

\begin{figure}
  %\vshrink{-0.4}
  \begin{center}
%\hspace{-0.62cm}
  \includegraphics[width=\columnwidth]{FIG/TBU.pdf}
%\vshrink{0.2}
  \caption{Overview of TBU.
  \label{fig:tbu}}
\end{center}
%\vshrink{0.6}
\end{figure}

\subsubsection{TCAM Banks}

Sequence alignment is search intensive since each sub-sequence 
coming from the measurement device has to be compared against 
potential indices of reference genome sequence. Hence,
we use TCAM arrays, which handles fast energy efficient
searches, as the base of our design. We store the reference genome 
in TCAM arrays and the sub-sequence under search in 
Shifting Logic Unit (SLU) of the TCAM. 
To make sure that the sub-sequence
is compared against the IFU-given indices of the reference genome,
SLU shifts the sub-sequence accordingly using SLU. 

\begin{figure*}[htp]
%\vshrink{0.7}
\begin{center}
%\hspace{-0.1cm}
  \subfloat[{\em full match}]{  
	\includegraphics[width=0.33\textwidth]{FIG/fullmatch.pdf}
		\label{fig:fullmatch}
 } 
 \subfloat[{\em right partial match}]{  
	\includegraphics[width=0.33\textwidth]{FIG/rightpartialmatch.pdf}
		\label{fig:partmatchright}
  }
 \subfloat[{\em left partial match}]{  
	\includegraphics[width=0.33\textwidth]{FIG/leftpartialmatch.pdf}
		\label{fig:partmatchleft}
  }
%  \vshrink{0.2}
  \caption{Possible match scenarios between the sub-sequence and the reference sequence stored in the array.
  \label{fig:match}}
\end{center}
%\vshrink{0.6}
\end{figure*}


To design the modified TCAM arrays, we first
take a look at an example. Figure~\ref{fig:match} depicts two match
scenarios. In one (Figure~\ref{fig:fullmatch}), the sub-sequence matches a
part of reference genome which is entirely stored in a single
row. We call this scenario a {\em full match}. However, in another
scenario (Figure~\ref{fig:partmatchright}), it is possible that the sub-sequence
matches a part of the reference genome which is stored in
two consecutive rows. In this example, the beginning part of
the sub-sequence (shown in green) matches the end of row j
while the rest of it (shown in red) matches the beginning of
next row row j+1 . We call this scenario a {\em partial match}. This
can happen at both ends of the SLU. If the remaining part of
the sub-sequence (red part) is on the right side of the SLU
(Figure~\ref{fig:partmatchright}), we call it a {\em right partial match}. Otherwise, as
shown in Figure~\ref{fig:partmatchleft}, it is called a {\em left partial match}.
TCAM arrays are already capable of finding all of the full
match scenarios among different rows. However, we need
extra hardware to find partial match scenarios as well. First,
to capture a {\em partial match}, we need to make SLU longer than
the length of a row. This way, it can compare a section of
the subsequence against the rows
% (as shown in Figures ??) 
as
well. If we see a match in such scenarios, we need to perform
an extra action to make sure that the rest of sub-sequence
matches the next or previous row. For instance in Figure~\ref{fig:partmatchright}
(Figure~\ref{fig:partmatchleft}), after a search operation found a right
(left ) partial match to row j , we need to compare the red part
of the subsequence to the beginning of next (previous) line,
row j+1 (row j−1 ). 
So, in a {\em partial match} case, search operation needs {\em \bf two} steps.

Besides, to improve energy efficiency of search operations, instead of searching
the whole bank for a match, we only search in specific rows. So, in a search operation,
only one row gets activated. Consequently, one Sense Amplifier (SA) gets activated and a MUX
at the end, selects the output of that SA to be fed to the Control Unit (CU) as the
{\em match signal}.




==> discussfig.tex <==
\begin{figure}[htp]
%\vshrink{0.7}
\begin{center}
%\hspace{-0.1cm}
  \includegraphics[width=0.9\columnwidth]{FIG/legend.pdf} \\
  \vshrink{0.5}
  \subfloat[Delay]{  
	\includegraphics[width=0.5\columnwidth]{FIG/micro17_pie_delay.pdf}
		\label{fig:piedelay}
 } 
 %\hspace{1cm}
 \subfloat[Energy]{  
	\includegraphics[width=0.5\columnwidth]{FIG/postmicro17_pie_energy.pdf}
		\label{fig:pieenergy}
  }
  \vshrink{0.2}
  \caption{Delay and energy consumption break-down for different units of BioCAM.
  \label{fig:discuss}}
\end{center}
\vshrink{0.6}
\end{figure}



==> discussion2.tex <==

[DISCUSSION2.TEX]

To see how having errors in prefix can degrade the outcome of
BioCAM, we quantify the probability of missing the alignment of 
a specefic base by BioCAM. 
BioCAM cannot align a base, when it appears in a query having
a substitution error in its prefix. 
Even worse, if the base
is changed due to mutation, BioCAM cannot align it, if the base itself appears
in the prefix region of a query. So, mutation-affected bases
lead to failure in alignment in both scenarios, which makes it
harder for BioCAM to align, compared to other normal bases.
Hence, we quantify what is the probability of not capturing
a mutation-affected base by BioCAM, as the worst case scenario. 
First, we quantify the probability
of missing this base when appeared in a random query, $P_{miss}$, which equals to
the probability of this mutation-affected base being in the prefix region,
or not being in the prefix region, but instead being in a query which has at least
a single substitution error in its prefix. Given 
$P_{sub\_err}$, probability of having at least a single 
substitution error in the prefix, equals to
$$1-(1-P_{NGS})^{prefix\_length},$$
we derive
$$P_{miss}=\frac{prefix\_length}{query\_length}+(1-\frac{prefix\_length}{query\_length})\times P_{sub\_err}.$$
$P_{NGS}$ denotes the probability of having substitution errors in a specific
NGS platform.
For a prefix length of 15 and query length of 100 (which is used in this 
study), $P_{miss}$ of
NGS platorms with $P_{NGS}=0.1\%$ ($P_{NGS}=1.0\%$) will be
nearly 16.3\% (26.7\%).

In real sequencing scenarios, each base is covered by multiple querys.
Coverage depth of querys is usually around 50\cite{ajay}, 
which means on average, each single base of the reference is 
covered by 50 different querys. Number of {\em query}s covering a base 
follows a Poisson distribution\cite{lander}.
Now,  considering the coverage depth, we want to quantify
the probability of a mutation being missed by BioCAM. 
In other words, we want to see
how probable it is that all the querys covering a single-base mutation 
are being missed by BioCAM.
To answer this, we first quantify what is
the minimum number of querys, expected to cover each base. 
For sequenced querys with
coverage depth of 50, based on Poisson distribution,
the probability of having a base that is covered by
only less than 10 querys is as low as $5.2\times10^{-12}$, almost zero. 
Given this, we assume each base is covered by at least 10 querys.
Now, even if
only 10 querys cover a mutation (which is very rare itself), 
the probability of missing alignment in all querys containing a mutation is 
$$(P_{miss})^{10}.$$
So, for NGS platforms with $P_{NGS}=0.1\%$ ($P_{NGS}=1.0\%$), the probability
of missing a mutation in all its querys becomes $1.3\times10^{-8}$ ($1.8\times10^{-6}$),
which is negligible.This becomes even more rare, when more number of 
querys cover the mutation, querys are longer than 100, or substitution
error rate of the NGS platforms improves further.
While all three of these are expected to happen in future NGS platforms, 
even considering the current technology which is used in this study,
we show that missing mismatches that happen in the prefix region does not degrade
the accuracy of BioCAM notabley.











==> discussionNew.tex <==
\vshrink{-0.1}
\noindent{\bf Errors in the {\em prefix}:}  Another source of inaccuracy is an
error in the \seed -long {\em prefix} used for search space pruning
(Section~\ref{sec:biocam}).  A corrupted {\em prefix} may lead to ill-addressed
search requests.  Let us start with the probability of \arch\ missing the
mapping to any given base within the {\em reference} due to errors in the {\em
prefix} of {\em query}s.  In practice,  more than one \ssq\ can contain, i.e.,
{\em cover} a given base of the {\em reference} genome.  The average number of
{\ssq}s covering any given base in the \srg\ is called {\em coverage} or {\em
depth} of sequencing.  \arch\ would miss the mapping to any base (of the {\em
reference)}, which is covered only by {\em query}s with a corrupted {\em
prefix}. NGS-induced (i.e., platform-dependent) substitution errors can corrupt
the {\em prefix}, and so can (platform-independent) mutations
(Section~\ref{sec:pr}).

Let us first quantify the probability of a given {\em query} missing a base of
the {\em reference} due to errors in the {\em query} {\em prefix}, $P_{miss}$.
$P_{miss}$ is the cumulative probability of having the {\em prefix} of the
respective {\em query} being corrupted by either at least one mutation-induced
substitution error, with a
probability of $P_{mut}$; or at least one NGS-induced substitution error, with a probability
of $P_{sub}$.  Per base character, let the probability of a mutation be $P_{M}$;
and the probability of an NGS-induced substitution error, $P_{NGS}$,  such that
%
%\vshrink{0.05}
%\noindent$$P_{sub}=1-(1-P_{NGS})^{prefix~length}$$
\noindent$$P_{mut}=1-(1-P_{M})^{seed}$$
\noindent$$P_{sub}=1-(1-P_{NGS})^{seed}$$
\noindent$$P_{miss}=P_{mut} + P_{sub}$$ %= P_{mut} + (1-P_{mut}) \times P_{sub}$$
%\noindent$$P_{miss}=\frac{prefix~length}{query~length}+(1-\frac{prefix~length}{query~length})\times P_{sub}.$$
%\noindent$$P_{miss}=\frac{seed}{query~length}+(1-\frac{seed}{query~length})\times P_{sub}.$$
%\vshrink{0.1}
%
\noindent applies, with {\em seed} denoting the {\em  prefix} length. 
%
In line with the evaluation, for {\em seed}=15, {\em query} length=100, and
$P_{NGS}=0.1\%$ ($P_{NGS}=1.0\%$) following Table~\ref{tbl:sa}, $P_{miss}$
becomes approximately 3.0\% (15.5\%). We set $P_{M}$ to 0.1\%, which is a widely
used estimate for mutation due to single-nucleotide
polymorphism~\cite{10002015global}.
%

Let us next quantify how $P_{miss}$ evolves with {\em coverage} depth, as more
than one {\em query} can cover a given base of the {\em reference}.  If we
assume a typical {\em depth} of around 50~\cite{ajay}, on average, 50 different
{\em query}s would cover each single base of the {\em reference}.  The number of
{\em query}s covering a base follows a Poisson distribution~\cite{lander}.  Let
us next derive the probability of \arch\ missing {\em all} {\em query}s covering
a respective base (of the {\em reference}) due to {\em prefix errors},
$P_{miss,all}$.  We first need to find the minimum number of {\em query}s
expected to cover each base.  Under Poisson distribution, and for {\em depth} =
50, the probability of having a base covered by less than 10 {\em query}s
becomes $5.2\times10^{-12}$, practically negligible.  Therefore, we can safely
assume that at least 10 {\em query}s cover each base.  Accordingly,
$P_{miss,all}$ becomes (${P_{miss}})^{10}$, which renders $5.9\times10^{-16}$
($8.0\times10^{-9}$) for $P_{NGS}=0.1\%$ ($P_{NGS}=1.0\%$). $P_{miss,all}$
would decrease further with increasing {\em coverage} depth and decreasing
$P_{NGS}$ as NGS platforms improve over time.  Therefore, even for the current
state-of-the-art, we do not anticipate notable accuracy loss due to {\em prefix}
errors.

Depending on the NGS platform, the {\em coverage} depth can be as large as 70 or
more~\cite{sims2014sequencing}.  Missing a small portion of {\ssq}s due to
different sources of system inaccuracies would be more tolerable under a higher
{\em coverage}, as the odds of encountering another {\ssq} to cover the missed
portion of the \srg\ increases.






==> discussionOld.tex <==
%probability of observing error in seed base-pairs is very low.
%
For instance, considering newer NGS platforms of Illumina \hl{(such as HiSeq
2500)} with an error rate of \hl{0.1\%}, and a
15-base-long {\em prefix}, this probability
becomes:
%of having
%error in 15 base pair is only 
$$1-0.999^{15}=1.5\%$$
%We neglect these errors to preserve the 
%We neglect missing the mapping of
%this small portion of requests to keep the 
%high throughput of \arch.

\hl{A workaround in this case is modifying the FilterU to detect potential matches
using} 
{\em similar} {\em prefix} 
\hl{values, as opposed to} 
{\em exact} 
\hl{(as it is the case for the default BioCAM implementation from Fig.}~\ref{fig:fu}\hl{).   
To match} {\em similar} {\em prefix} \hl{values, if we only account for a substitution error of one base in a 15-base-long
}
{\em prefix}
\hl{as an example,
FilterU would need to consider 
}
 $$3 \times 15 = 45$$
 \hl{different options for each}
{\em prefix} \hl{value. This is because the substitution error can occur at any of the 15 base-positions,
  by substituting the respective base with any of the 3 remaining base values from
  the 4-base alphabet.
This translates into} 
$45\times$ 
\hl{more operations, which apply to}  1.5\% (14.0\%) \hl{of the} {\ssq}\hl{s (that would not find a match otherwise) under a
substitution error rate of} 0.1\% (1\%), \hl{respectively.
  The resulting slow-down for the} 0.1\% (1\%) \hl{error rate can reach} 
$1.65\times$
($7.3\times$), \hl{reducing BioCAM's throughput improvement over Barracuda to around}
$4.5\times$ ($1.03\times$).
%
\hl{The substitution error rate of}
1\% \hl{corresponds to older NGS platforms (such as Illumina Genome
Analyzer), and NGS error rates are expected to decrease, not increase (similar
to improvements due to technology scaling under Dennardian scaling, before
stagnation).
The proof-of-concept BioCAM implementation neglects these errors, assuming the more representative error rate of 0.1\%.
}


\ignore{To avoid these errors, we should consider potential
substitution errors in the {\em prefix}. To do so, we need to search for
potential matches using similar {\em prefix}. For instance, if we only
consider one base substitution error in a 15-base-long {\em prefix},
$$3 \times 15 = 45$$
similar {\em prefix} should be searched (as opposed to one), because each base can be
substituted by 3 different values due to an error.
Under a substitution
error rate of 0.1\% (1\%),
this translates into $45\times$ more search operations on average
for 1.5\% (14.0\%) of the \ssq s (that will not find a match otherwise).
%, on average,
%$45\times$ more search operations are needed in order to 
%capture similar {\em prefix}s. 
The resulting slow-down for the 0.1\% (1\%) error rate can reach $1.65\times$ ($7.3\times$).
%This 
%will diminish all the initial 
%benefits observed using BioCAM. While missing this amount of
%\ssq s is already tolerarble in Bioinformatics domain (Barracuda
%misses XXX\% of the \ssq~s) and substitition error is as low as 0.1\%
%\hl{in recent NGS platforms, 
We neglect such errors to preserve the
high throughput of \arch, under the more representative error rate of 0.1\%.
%BioCAM does not consider substitution errors in
%{\em prefix}.

\hl{
%For NGS platforms with larger error rates, this probability increases.
Substitution error rate for some older popular Illumina NGS platforms (as depicted in
Table}~\ref{tbl:sa}\hl{) is
around 1\%. In this case, probability of error in a 15-base-long }{\em prefix}\hl{
can reach 14.0\%.
%Still, this is acceptable in bioinformatic domain. [WE CAN ASK MEISAM
%TO COMMENT ON THIS.] }
However, NGS error rates are expected to decrease, not increase (similar to
  improvements due to technology scaling under Dennardian scaling, before
  stagnation).
%(2) We can change the search logic to work with similar prefix.
}

}


==> evalfig-asplos.tex <==
\begin{figure*}[h]
%\vshrink{0.7}
\begin{center}
\hspace{-1cm}
\begin{minipage}{0.28\textwidth}
	\includegraphics[width=\columnwidth]{FIG/micro17_safp.pdf} 
	%\caption{False positive probability vs. {\em tolerance} overshoot.}
	\caption{{\em Less similar match} probability vs. {\em tolerance} overshoot.}
	\label{fig:sa} 
\end{minipage}
\begin{minipage}{0.65\textwidth}
  \subfloat[Throughput Performance]{  
	\hspace{0.25cm}
	\includegraphics[width=0.5\textwidth]{FIG/postmicro17_throuput_combined.pdf}
		\label{fig:throughput}
	\hspace{0.25cm}
 } 
 \subfloat[Energy]{  
	\includegraphics[width=0.5\textwidth]{FIG/energy_postmicro17_combined.pdf}
		\label{fig:energy}
  }
  \vshrink{0.1}
  %\caption{Throughput performance and energy consumption of a single \arch\ DIMM.
  \caption{Throughput performance and energy consumption.
  \label{fig:eval}}
\end{minipage}
\end{center}
\vshrink{0.4}
\end{figure*}



==> evalfig-isca18.tex <==
\begin{figure}[h]
%\vshrink{0.2}
\begin{center}
  \includegraphics[width=0.45\textwidth]{FIG/isca18/legend2.pdf}\\
  \vshrink{0.2}
  \subfloat[Throughput Performance]{  
%	\hspace{0.25cm}
	\includegraphics[width=0.45\columnwidth]{FIG/isca18/isca18_throughput.pdf}
		\label{fig:throughput}
%	\hspace{0.25cm}
 } 
 \subfloat[Energy]{  
	\includegraphics[width=0.45\columnwidth]{FIG/isca18/isca18_energy.pdf}
		\label{fig:energy}
  }
  \vshrink{0.1}
  %\caption{Throughput performance and energy consumption of a single \arch\ DIMM.
  \caption{Throughput performance and energy consumption.
  \label{fig:eval}}
\end{center}
\vshrink{0.4}
\end{figure}



==> evalfig-old.tex <==
\begin{figure*}[h]
%\vshrink{0.7}
\begin{center}
%\hspace{-0.1cm}
  \subfloat[Throughput Performance]{  
	\includegraphics[width=0.3\textwidth]{FIG/postmicro17_throuput_combined.pdf}
		\label{fig:throughput}
 } 
\hspace{0.25cm}
 \subfloat[Energy]{  
	\includegraphics[width=0.3\textwidth]{FIG/energy_postmicro17_combined.pdf}
		\label{fig:energy}
  }
  \vshrink{0.1}
  %\caption{Throughput performance and energy consumption of a single \arch\ DIMM.
  \caption{Throughput performance and energy consumption.
  \label{fig:eval}}
\end{center}
\vshrink{0.4}
\end{figure*}



==> evelfig.tex <==
\begin{figure*}[htp]
%\vshrink{0.7}
\begin{center}
\hspace{-0.1cm}
  \subfloat[throughput]{  
	\includegraphics[width=0.5\textwidth]{FIG/micro17_throuput_combined.pdf}
		\label{fig:throughput}
 } 
 \subfloat[energy]{  
	\includegraphics[width=0.5\textwidth]{FIG/energy_micro17_combined.pdf}
		\label{fig:energy}
  }
  \vshrink{0.2}
  \caption{Throughput and energy consumption of a single BioCAM dimm.
  \label{fig:eval}}
\end{center}
\vshrink{0.6}
\end{figure*}



==> fixme.tex <==
-------------------------------------------------------------------------------
-------------------------------------------------------------------------------

- abs.tex: introduce similarity?

- shall we spell out "short reads"?

- single-end vs. double(pair)-end alignment? 

- Trend: increased read length and more errors ("permitted in final alignment").
  It is not clear what the latter means: more errors expected or twd similarity
  search?

- there are 3 types of alignment errors: insertion, deletion, substitution

- PMIT  organized as a TCAM? Add to future work?

- how to justify that we are only comparing against BarraCUDA?

- can we say that we are "hardcoding" the scoring into the TCAM array by the
  similarity search mechanism?

- can we quantify scalability?

- ~\cite{hybridAccFPGA} provides code. Have to include.

- call m "seed length"?

-------------------------------------------------------------------------------
-------------------------------------------------------------------------------

- Why not bases but base pair?

- How is a genome defined wrt a DNA strand? 

- Is the non-denovo sequence assembly problem we are tackling more
  important/harder indeed?

- There are 4 types of alignments for each base, namely exact match, mismatch,
  insertion and deletion. We do not tackle these in the way BarraCUDA is doing.

-------------------------------------------------------------------------------
-------------------------------------------------------------------------------


==> hierarchy.tex <==
\noindent
Our focus so far was on the basics of \arch's mapping mechanism.  We will next
look into mapping accuracy, and specifically identify under what circumstances \arch\
would fail to map a given {\em query} to the respective {\em reference}, which
in fact was {\em similar enough}.
%
As explained in Section~\ref{sec:pr}, the most likely reason is reverse
complement of {\em query}s, since NGS platforms typically sequence almost half of
the DNA strands in reverse order.  The next likely reason is having substitution
mismatches 
\redHL{(the dominant type of mismatches) [XXX this is necessary 
to understand why this is the next likely reason]}
in the \seed-long {\em prefix} used for search space pruning
(Section~\ref{sec:biocam}).
%, be it NGS platform-induced or SNP.  
A corrupted {\em
prefix} may lead to ill-addressed search requests, i.e., FilterU sending
incorrect PMIs to MatchU.  Finally, the least likely reason is 
%a short indel in
\redHL{having indels anywhere}
the {\em query}, since TCAM arrays can only handle substitution errors. 
Other \redHL{less likely [XXX: or even rare]} reasons might be 
due to the existence of complex repetitive regions or 
complex genome variations which are very challenging to detect and is beyond 
the scope of this work.

\arch\ employs multi-phase hierarchical mapping, where each phase acts as a
filtering layer for the next phase which in turn performs more sophisticated
mapping, considering only the subset of {\em query}s the previous phase failed
to map.  In other words, a phase re-attempts mapping only for the subset of {\em
query}s that the previous phase failed to map. 
%Specifically, in each of the above cases, 
If the mapping in a phase fails, MatchU raises the {\em Failed-Map} signal.
\arch\ in turn feeds {\em Failed-Map} back to FilterU, to trigger  more
sophisticated mapping attempts in the subsequent phase(s), as need be. 
%The
%default, i.e., the first phase, performs mapping considering platform-induced
%substitution errors and SNPs only (except in the {\em prefix}).  

To handle failed mappings due to reverse complement of {\em query}s, 
%the first issue, 
after getting {\em Failed-Map} from MatchU (at the end of the first phase),
FilterU immediately sends PMIs corresponding to the reverse complement of the
{\em query} to the MatchU. To accelerate this process, MatchU employs an extra
register inside the Shift Logic, which keeps the reverse complement of the {\em
query} in addition to the original.  MatchU copies the reverse complement in
this register at the time it gets 
%in parallel with storing 
the original {\em query} (during the first phase).  Therefore, upon receipt of
{\em Failed-Map}, FilterU does not need to broadcast the reverse complement of
the {\em query} separately, but only the PMIs for the reverse complement (which
FilterU simply extracts by consulting the PMI tables with the \seed-long {\em
prefix} of the reverse complement of the {\em query}).
%of the {\em query}. 
%
Attempting mapping for reverse complements hence forms \arch's second phase for
mapping.

If the second phase fails to map the {\em query}, as well, we are left with
three possibilities: (i) there are 
%(substitution) 
mismatches in the {\em prefix};
(ii) there are indels anywhere in the {\em query} (since TCAMs cannot detect
them); or (iii) the {\em query} simply is too unsimilar to the {\em reference}
due to too many mismatches.  
Unfortunately case (iii), which is typically due to complex genome variations, 
is very challenging to fix. However, these variations are rare. 
%No mapping algorithm can handle (iii), which luckily is
%rare. 
To address the first two cases,
\redHL{following well-known {\em anchoring} techniques~\cite{bowtie1}},
\arch\ chunks the {\em query} into two
halves, and re-attempts mapping each half separately in two subsequent phases.
Such \redHL{anchoring} is promising 
as mismatches to result in a failed mapping are less
likely to occur in shorter {\em query}s. After these two phases, in case of
failure in alignment, \arch\ attempts to align reverse complement of the two
halves as well.

%(i) has a higher probability than
%(ii).  Therefore, 
%Mapping only the first half of the {\em query} helps to align 
%when the full {\em query} contains indels in the second half.
%On the other hand, mapping the second half of the {\em query}
%(which excludes the {\em prefix} considering typical \seed\ values and {\em
%query} lengths), and then the first half only (which includes the {\em
%prefix} considering typical \seed\ values and {\em query} lengths).
%FilterU always loads PMIT address ranges corresponding to the next
%step from PMITIL, to accelerate these phases.

In Section~\ref{sec:acc}, we will quantify how \redHL{anchoring} can improve
mapping accuracy significantly. However, \redHL{anchoring} is helpless 
if \arch\ fails to align both halves of the {\em query}.
\arch\ could fail to map a {\em query} under two 
scenarios: due to mismatches in the {\em prefix} or having indels anywhere.
Let the probability of having mismatches in the {\em prefix} of a {\em query} be
$P[\textit{mismatch~in~prefix}]$, and the probability of having indels
in a {\em query} be
${P[\textit{indels~in~query}]}$.

Let $P[\textit{mismatch}]$ be the per base probability of a mismatch, 
be it due to NGS platform or genome variations.
Then,
$$P[\textit{mismatch~in~prefix}]=1-(1-P[\textit{mismatch}])^{seed}$$
applies. 
We can estimate $P[\textit{mismatch}]$ by adding NGS platform %substitution
error rate, 0.1\%~\cite{insdel}, and average genome variation rate, 0.1\%~\cite{var1,var2,var3}.
Using this  estimate, for a representative \seed\ value of 15 (Section~\ref{sec:setup}),
$P[\textit{mismatch~in~prefix}]$ barely reaches 3.0\%.

The most common indel-type variations are short indels, induced by genome variations  
(other indel-type variations are rare).
Let $P[\textit{indel}]$ be the probability of a short indel, and $l$, the length of a {\em
query}. Then,
$$P[\textit{indels~in~query}] = 1-(1-P[\textit{indel}])^l$$
applies. 
While there is no exact consensus on the rate of short indels, 
different studies estimate the expected probability of short indels 
based on the observed previous cases~\cite{var1}. 
For example, the work \cite{var5} identifies 
%$\approx 3$ millions SNPs and 
$\approx 135K$ short indels in the sequenced genome (which is of size $3$ billion). 
Let us, for the sake of illustration, use the conservative 
choice of $0.01\%$ for $P[\textit{indel}]$. 
Using this estimate, for a representative query length of $150$~\cite{illumina}($l = 150/2 = 75$), 
${P[\textit{indels~in~query}]}$ barely reaches $1.0\%$. 

\ignore{
Different studies estimate the expected
probability of short indels as approximately 1/11$^{th}$ of the genome variation
rate~\cite{var1,var2,var3}. Hence, 0.009\% is a viable estimate for $P[indel]$. 
Using this estimate, for a representative {\em query} length of 150~\cite{illumina}
($l=150/2=75$),
$P[\textit{indels~in~query}]$ barely becomes 0.7\%.
}

We can estimate the probability of \arch\ failing to align a half,
by adding $P[\textit{mismatch~in~prefix}]$ and ${P[\textit{indels~in~query}]}$,
which is around 4.0\%. Then, probability of \arch\ failing to align both halves becomes
$(4.0\%)^2 \approx 0.16\%$.

\ignore{
of a given {\em query, q}, but where the {\em prefix} of the second half
of {\em q} also has errors. Let the probability of this scenario be 
%$P_{double err,{prefix}\times 2}$.  
%$\texttt{
  $P[\textit{prefix~error~in~all~chunks}]$.
  %}$.  
The second one is, if indels exist in {\em
both} halves of the respective {\em query}. Let the probability 
%of this scenario
be 
%$P_{err_{indel}\times 2}$.
${P[\textit{indels~in~all~chunks}]}$.
%{\em P[indels in all chunks]}.
%

Let $P[\textit{substitution}]$ be the probability of a substitution, be it due to a
platform-induced error or SNP. Then, 
$$P[\textit{prefix~error~in~all~chunks}]=(1-(1-P[\textit{substitution}])^{seed})^{\#chunk}$$
applies, with chunk count $\#chunk=2$, as the \seed\ value does not change
across phases.  The substitution error probability of a representative
modern Illumina platform is reported as around 0.1\%~\cite{insdel}. Besides, 0.1\%
is a well-accepted estimate for the SNP
probability~\cite{var1,var2,var3}.  We can calculate $P[\textit{substitution}]$ by adding
these two probabilities. Using this estimate, for a representative {\em seed} value of 15 (Section~\ref{sec:setup}),
$P[\textit{prefix~error~in~all~chunks}]$ barely reaches 0.09\%.

Let $P[\textit{indel}]$ be the probability of a short indel, and $l$, the length of a {\em
query}. Then,
$$P[\textit{indels~in~all~chunks}] = (1-(1-P[indel])^{l/{\#chunk}})^{\#chunk}$$
applies, with chunk count $\#chunk=2$. 
Different studies estimate the expected
probability of short indels as approximately 1/10$^{th}$ of the SNP
probability~\cite{var1,var2,var3}. Hence, 0.01\% is a viable estimate for $P[indel]$. 
Using this estimate, for a representative {\em query} length of 150~\cite{illumina},
$P[\textit{indels~in~all~chunks}]$ barely becomes 0.006\%.
}

Without loss of generality, the proof-of-concept \arch's
\redHL{anchoring} implementation adapts
2-way chunking, where multi-way (and not necessarily uniform) chunking can
further help reduce the number of failed mappings. We leave the exploration of
this rich design space to future work.
%
Through \redHL{anchoring}, 
the probability of missing a mapping can significantly reduce,
but depending on the application, this may still not be good enough.
To cover
such cases, \arch\ and software implementations of sophisticated high-overhead
algorithms can be paired as follows: If after multi-phase attempts \arch\ fails
to map some {\em query}s, it stores them in a dedicated memory location, over
DMA, for the software to read and process. 
Highly optimized software
packages (such as~\cite{luo2013soap3}) already commonly rely on similar multi-phase
refinement. 
\redHL{
Besides, to get SAM format output for the aligned queries, 
\arch\ sends the final matching indices to this software, as well, to find
different SAM format fields such as CIGAR and MAPQ.
%Although negligible (due to the very low likelihood), 
We will quantify the
overhead of this hardware-software hybrid solution, $BioMAP++$, 
in Section~\ref{sec:eval}.
}
%

%%%%%%%%%%%%%%%% BEGIN MEISAM
Putting it all together, let us conclude this section with a thought experiment:
Let us assume that there are two algorithms $A_{sub}$ and $A_{indel}$ for
mapping {\em read}s to the {\em reference} genome. While $A_{sub}$ can handle
substitution errors only with time $t_{sub}$ per {\em read}, $A_{indel}$ can
handle both substitution and indels in time $t_{indel}$. Also assume that
$t_{sub} \ll t_{indel}$. This is generally true since handling indels is much
more difficult than substitution errors. Let us define a new meta-algorithm
which uses algorithm $A_{sub}$ for each {\em read} and only if the {\em read}
cannot be mapped, passes the read to the next phase algorithm $A_{indel}$.  
Then we can give the run time of the
algorithm approximately by
%
$$\max( n \times p_{indel} \times t_{indel}, n \times t_{sub})$$
%
where $n$ is the total number of {\em read}s and $p_{indel}$ is the probability of
indels.
Since $p_{indel} \ll 1$ and $t_{sub} \ll t_{indel}$, this meta algorithm can lead to huge
computational savings when compared to $A_{indel}$ which requires $n \times t_{indel}$. 
This simple thought experiment illustrates the time saving resulted from the hierarchical alignment structure.  

From a statistical point of view, one might argue that using $A_{sub}$ first and
$A_{indel}$ next might cause statistical loss when a {\em read} gets mapped with $A_{sub}$
while it could have been mapped with $A_{indel}$ with higher likelihood. We can
  avoid this
  loss by setting a threshold for the number of
  acceptable substitution errors in $A_{sub}$ carefully. Let us use $p_{indel}$
  and $p_{sub}$ to denote the indel and substitution probability, respectively.
  Then we just need to only accept mappings in $A_{sub}$ with
  $\log(p_{indel})/\log(p_{sub})$ number of substitutions or less. This threshold
  guarantees that any sequence is mapped to the location (in the {\em
  reference}) with largest
  likelihood for similarity. In the worst case, we can always set the threshold for the number
  of acceptable errors in $A_{sub}$ to one, which prevents statistical loss
 due $p_{indel}\ll p_{sub}$.  
 \redHL{[MEISAM: do you think we need to add the rebuttal discussion here?]}
% \vshrink{0.2}
 %The GPU solution from Luo et. al.~\cite{luo2013soap3} employs a simili
 %However, as we will see in Section~\ref{sec:eval},
 %it is possible for even larger values of the threshold not to cause any
 %practical statistical loss, as well.
%%%%%%%%%%%%%%%%% END MEISAM


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{
To improve accuracy and alignment rate, \arch employs a hierarchical search
approach to align the {\em query}s that could not be aligned.  As explained in
Section~\ref{sec:pr}, the most potential reason for unalignment is reverse
complement issue, since NGS platforms reads almost half of the DNA strands in
reverse order.  Next most common issue is dealing with substitution errors that
may appear in the prefix, being a NGS platforms induced substitution error or a
mutation induced variation. In this case, FilterU will send a wrong list of PMIs
to the MatchU, leading to unalignment.  Finally, unalignment can be a reason of
rarely having short indels in the {\em query}, since TCAM arrays can only handle
substitution errors.

To handle the first issue, after getting an unalignment signal from MatchU,
FilterU immediately sends PMIs corresponding to the reverse complement of the
{\em query} to the MatchU. To accelerate this process, MatchU employs an extra
register inside the Shift Logic, keeping the reverse complement of the read, as
well as the original one.  MatchU stores the reverse complement in this register,
in parallel with storing the original {\em query}.  So, FilterU does not need to
broadcast the reverse complement of the {\em query} separately.  Besides, after
loading all PMIs of the original {\em query} from PMIT which is shorter than
searching for all of them in MatchU, FilterU immediately loads PMIT address
range of the reverse complement of the {\em query}, and keeps it in a temporary
register. Hence, in case of receiving a unalignment signal, it can immediately
load the corresponding PMIs from PMIT.

If still MatchU cannot align a {\em query}, it is either due to having errors in
the prefix, having indels anywhere (since TCAMs cannot detect them), or {\em
query} being too unsimilar to the {\em reference} to detect, due to too many
errors.  In the last case (which is rare), all mapping platforms will fail to
align.  To address the first two cases, \arch employs an anchoring technique, in
which it searches for a subset of the {\em query}. This helps aligning the
reads, since probability of having errors in both halves of a {\em query} that
can lead to unalignment is lower, in shorter {\em query}s.  Having errors
(including NGS platform induced and SNPs) in the prefix is more common compare
to having indels. So, \arch first searches for the second half of the {\em
query}, and then for the first half only.  Like handling reverse complements, to
accelerate this process at each step, FilterU always loads PMIT address ranges
corresponding to the next step from PMITIL.

While we show in Section~\ref{sec:evalaccur} how anchoring improves 
accuracy significantly, it may still fail to resolve two scenarios.
When unalignment is due to having errors in the prefix, anchoring will fail
if errors exist in the prefix of the second half of the {\em query} as well.
We call the probability of seeing this scenario $P_{err_{prefix}}$.
Furthermore, anchoring fails when there are indels in both halves of the {\em query}.
$P_{err_{indels}}$ quantifies the probability of the second scenario.

Assuming $P_{var_{base}}$ being the probability of having variation in a base
(being NGS platform or mutation induced), $$P_{err_{prefix}} =
(1-(1-P_{var_{base}})^{seed})^2.$$ For a modern Illumina NGS platform,
substitution error rate is around 0.1\%[???].  Besides, for average
mutation-induced variation rate 0.1\% represents a well-accepted number[???].
We can estimate $P_{var_{base}}$ by sum of these two rates. Then, for a {\em
seed} value of 15 (a representative number), $P_{err_{prefix}}$ is only around
0.09\%.

Assuming $P_{indel}$ being probability of having an indel in a base, and $QLEN$
being length of the {\em query}: $$P_{err_{indels}} =
(1-(1-P_{indel})^{QLEN/2})^2.$$ $P_{indel}$ is usually one tenth of the total
mutation-induced variation rate[???], approximately 0.01\%. Then, for a {\em
query} length of 150 (a representative number), $P_{err_{indels}}$ is only
around 0.006\%.

While these failure rates look negligible, still there might be a scenario that one might
want to handle these cases as well. After the hierarchical search, if \arch still
could not align some {\em query}s, it stores them in a dedicated memory location, over DMA.
Then, in a post-processing step, a more expensive software-based read mapping platform can be
used to map the remaining unaligned {\em query}s. 
Although negligible, we quantify this overhead
in Section~\ref{sec:eval}.
}


==> hiertbl.tex <==
%\begin{table}[tp]
\vshrink{0.1}
\begin{table}[h]
\centering
\caption{Probability of missing a mapping for Phase 1.}
\label{tbl:hier}
\vshrink{0.1}
\begin{tabular}{l||c|c|c}
\textbf{Case}      & Reverse complement &  {Prefix} corruption & Indels  \\ \hline 
\textbf{Probability} & $~ 50\%$           & $3.0\%$               & $1.5\%$
\end{tabular}
\vshrink{0.2}
\end{table}


==> intro.tex <==
% intro.tex

** In BioCAM, all base-pair (bp) differences are considered similarly. For instance,
it does not matter whether we have 3 bps difference besides each other, or
scattered in 3 different locations apart from each other. Finding burst of
differences is challenging for existing sequence alignment applications.
However, BioCAM detects such cases without any extra effort.
\redHL{what is a ``burst of differences''? is the above a + or a - trait of
\arch?}

** \arch\ can search the whole reference genome energy-efficiently. So, it
can find as many similar aligning indices as possible. Finding all similar
parts of a reference genome is challenging for existing algorithms since
they usually rely on early-termination after finding the first match.
\redHL{need to detail + quantitative motivating example}




==> mdevtbl.tex <==
\begin{table}[tp]
\centering
\caption{Average coverage rate for difference number of bps.}
\label{tbl:mdev}
\begin{tabular}{lccc}
\textbf{\# of bps} & \textbf{5} & \textbf{10} & \textbf{15} \\ \hline
No SGU             & 95.1\%     & 90.4\%      & 86.0\%      \\
single-bp SGU      & 99.9\%     & 99.6\%      & 99.0\%     
\end{tabular}
\end{table}


==> motiv.tex <==
\redHL{merge w/ Intro?}

In this section, we explore key insights needed to design an accelerator based
on the proposed TCAM designs such as \redHL{[cite Engin papers here]}. As we have seen
in Section  \redHL{[background? or a separate one for ``problem statement''?]},
sequence alignment finds a match, when two sequences are {\em almost} similar.
Existing TCAM implementations are not able to find similar patterns. Instead,
they can find {\em exactly identical} patterns with high energy-efficiency.
Thus, we propose modifications to the existing array designs in Section
\redHL{[background?]} in order to enable {\em similarity matching} in TCAM arrays.

Next we take a look at a case study, comparing an implementation of sequence alignment
using existing TCAM solutions and a representative GPU solution, at a high level.
\redHL{make the case that these TCAM solutions are ``representative''}
We rely on the latest version of BarraCuda \redHL{[BarraCuda]} as one state-of-the-art
sequence alignment on GPGPUs.
\redHL{BarraCuda: can we safely say ``best-known''?{\bf (We should consult Meysam here.)}}

{\bf Case Study:} Neglecting the fact that existing TCAMs are unable to capture {\em similarity},
we assume that we use the most energy efficient design of a representative study \redHL{[Engin]} for 
sequence alignment. 
\redHL{where would UCSD work fit?}
In this study, search operations are energy efficient and fast, consuming
only 245nJ to search for a pattern in all rows of a $1K\times 1K$ array 
(the most energy and area efficient design presented in [engin]) in 2.5ns.
\redHL{are these numbers directly coming from the paper or derived? if the
former applies, can cite a table or figure. {\bf (Yes these are directly extracted
from Table3 of that paper.)}}
\redHL{Need insight for why 1Kx1K is representative, and a discussion at the end
of this case study for how the picture would change if we had a different array
layout and/or size {\bf (added to the text)}}
A human genome contains near 3Gbps. We assume each bp is represented with 2 bits,
 which is simply the minumum number of bits needed to encode 4 different bps,
 leading to the least possible number of arrays needed.
\redHL{justification?{\bf (added to the text)}}
Then, we need approximately 6K arrays to keep the whole reference genome.
\redHL{shouldn't this be 6K? Otherwise use the more accurate value for 3Gbp?
Also, we have to make sure that this is not mistaken for the ``database''
content in the proposed design.{\bf (updated the text accordingly)}}
Besides, to search a given sub-sequence against all possible locations of the reference genome,
we need to shift it at least 512 times per array\footnote{The real number is 512 + length of
the given sub-sequence. We neglect the later for simplicity, without affecting the conclusion}.
\redHL{shouldn't we talk about expected lengths here? may be presented in the
backgnd, but a careless reader may get lost still; it is not clear based on the
information provided in this Section so far where these shifts are coming from,
and why particularly 512.}
This means to search the whole reference genome for potential matches to a given sub-sequence,
512 search operations per each of the 5700 arrays should be done. Recalling energy consumption
per search in a single array (245nJ), to align a single sub-sequence using existing TCAM array
designs, at least 
$$6000 \times 512 \times 245nJ = 752.6mJ$$
of energy is consumed.

On the other hand, existing GPGPU solutions such as Barracuda are shown in [Barracuda] 
to be able to
align 16000 sub-sequences per second on average, on a Tesla K40 GPU node, with TDP of 235W.
\redHL{Is there anything specific about Tesla K40?{\bf (updated the text, 
this is what they have used)}}
Even at peak power, aligning each sub-sequence consumes
$$\frac{235J}{16000}=14.7mJ$$ of energy, which is $51.2s\times$ more energy efficient
than TCAM-based implementation. So, 
even a high-level analysis (favoring the TCAM-based) shows that a sole mapping of alignment
problem to existing TCAM arrays is not sufficient.
\redHL{How about the UCSD work as an ``existing'' TCAM array?
{\bf (It is perpendicular to this study as a comparison work)}}


TCAM arrays are shown to be significantly more energy efficient in comparison to general-purpose
processors. Thus, this large energy efficiency gap shows a fundamental implementation difference.
Barracuda runs on a transformed genome which is generated in a pre-processing step. 
This transformed genome helps in searching
for a given sub-sequence in a pruned space, instead of aligning to all 3Gbp locations. 
Hence, orders of magnitude less number of operations are needed per sub-sequence in
Barracuda's implementation compared to the aforementioned TCAM-based one, leading
to higher energy efficiency benefits.
\redHL{Let us call this TCAM-based solution ``Naiive''. This is also a good way
of providing the background on BarraCuda, instead of confining it to the backgnd
section which readers may skip.{\bf (Agreed!)}}

Based on these observations, we introduce BioCAM, an alignment accelerator based on TCAM arrays.
In \arch, TCAM arrays are modified to enable searching for {\em similarity} rather than exact
match only. Besides, an efficient filtering mechanism prunes the search space, leading
to a more energy-efficient solution compared to Barracuda.




==> notes.tex <==
%\input{introNew}
%\input{notes}
%\input{intro}
%\input{relMicro}

** In BioCAM, all base-pair (bp) differences are considered similarly. For instance,
it does not matter whether we have 3 bps difference besides each other, or
scattered in 3 different locations apart from each other. Finding burst of
differences is challenging for existing sequence alignment applications.
However, BioCAM detects such cases without any extra effort.
\redHL{what is a ``burst of differences''? is the above a + or a - trait of
\arch?}

** \arch\ can search the whole reference genome energy-efficiently. So, it
can find as many similar aligning indices as possible. Finding all similar
parts of a reference genome is challenging for existing algorithms since
they usually rely on early-termination after finding the first match.
\redHL{need to detail + quantitative motivating example}

\begin{small}
\begin{verbatim}
[Problem Statement]
- "Short" Read Sequence Alignment
- Next generation DNA sequencing (NGS) renders a thorughput of 600Gba per instrument
  run. This is 200 times the depth of coverage of the human genome.
  --> an enormous amount of sequence data is available
- Baseline for comparison: A GPGPU sequence alignment software: 
"based on BWA, to accelerate the alignment of sequencing reads generated by
these instruments to a reference DNA sequence."
- Challenges and opportunities for hardware acceleration?
- Sequencing: NGS output lengths range from ("short sequencing reads") 25 to 400 bps.
--> what do we assume? Sensitivity analysis>
\end{verbatim}
\end{small}


\begin{small}
\begin{verbatim}
[Motivation]
1. Why NV TCAM?
  + A CMOS (charged-based) TCAM cell is relatively large: 
	3.8xSRAM; over 90xDRAM
  + Immunity to transient errors
  + Practically 0 leakage power
  - Write endurance (PCM), latency
  - Slow reads (PCM)
\end{verbatim}
\end{small}


\begin{small}
\begin{verbatim}
[System Integration]
- Fig.2 from~\cite{ipekTCAM}
- Communication overhead within a DIMM?
- Recall that~\cite{ipekTCAM} includes a discussion for DDR3 compatibility,
  which may be overkill for bioCAM: since DDR would try to collect the results 
  earlier than a search might finish (following the read convention), dummy
  writes need to be added. To mitigate the adverse impact on the DDR bus,
  pipelining is proposed to overlap search and reduction phases particularly. In
  the context of BioCAM, processing multiple sequence may lead to natural
  pipelining. 
- Implications/adaptation to 3D stacking?
- How about connection over the PCI bus?
\end{verbatim}
\end{small}


\begin{small}
\begin{verbatim}
[TCAM design]
- To avoid additional transistors, writes are performed in a sequential fashion
  (the number of transistors which can be programmed at a time is
  limited)~\cite{ipekTCAM}. This is likely to improve density~\cite{ipekTCAM}.
  For BioCAM, the performance trade-off is likely to be invisible as the TCAM is
  not write heavy.
  - Rows can be disabled entirely. Also, matchlines are segmented (and wider
	searches are performed in series by holding the partial results)
	~\cite{ipekTCAM}.  
\end{verbatim}
\end{small}


\begin{small}
\begin{verbatim}
[Sources of Errors]
- PCM's variability and limited write endurance (the latter is mostly irrelevant
  as the TCAM is not often written in this case)
- Machine read errors
- Mutation
\end{verbatim}
\end{small}


\begin{small}
\begin{verbatim}

[Misc]

- Sequence homology detection or sequence alignment is a computationally
  expensive operation which finds place in almost all bioinformatics sequence
  analysis applications. There is an inherent scalability problem as sequence
  databases are growing exponentially. Growth rate estimations? Pure function of
  sequencing capabilities?

- Three options:
* One to one: Pair-wise sequence alignment (PSA), e.g., SW
** One to many: A sequence is searched against a database of many sequences,
   e.g., BLAST 
*  Many to many: Multiple sequence alignment (MSA)
Parallel variants of all algorithms exists.
Are these serving different purposes, or are these evolve as a function of
sequencing capabilities -- i.e., can each regarded be as a generalization of the
former?
In all, the sequence can be a DNA or protein sequence. The algorithms are
dominated by integer operations. SA is data-intensive.

\end{verbatim}
\end{small}


\begin{small}
\begin{verbatim}

[Opens]

- Similarity metric not clear?
  
  Mutation and noisy machine reads matter in this context. We model these as
  abstracted out noise probabilities.

- The current implementation (at the high-level) pretty much looks like a BLAST
  variant...

- Iso-alignment fidelity?

  BioCAM is always better.

- Problem statement: Exact vs. inexact alignment -- mismatches and full-gapped
alignment... There are 4 types of alignments for each base, namely exact match,
mismatch, insertion and deletion.
It is not clear how we tackle the latter two.

- Baseline for comparison: which portions of the algorithm are exactly being
accelerated?

- Metric for evaluation: Throughput performance, energy efficiency, at
*iso-alignment fidelity*

\end{verbatim}
\end{small}


\ignore{
In computational molecular biology, finding the optimal alignment between two
DNA sequences is a key step in identifying shared ancestry, and thereby,
functional impact of genes.

" ... Any sequence similarity can then be used to infer function and evolutionary
 relationships.  In fact, one common method for examining and comparing genes is
 to search for similarities between newly sequenced DNA and databases of gene
 sequences that have already been described. By identifying related genes or
 gene families with known functions, scientists can infer the functions and
 evolutionary relationships of newly cloned genes or even whole genomes."

- Problem statement: definition, importance of sequence alignment
- State of the art
- Bottlenecks
- Proposed solution
- Paper Roadmap

- NGS machines got faster, operating at a very high throughput

- The result was an huge amount of search data

- Sequence alignment is one of the first steps for analysis of this data. 

- During SA, sequencing reads get mapped to other reads to form a genome (de
novo sequence assembly) or on to a reference DNA sequence.
"BarraCUDA p.27: sequence alignment is one of the first steps for downstream data analyses,
during which sequencing reads have to be mapped either to other reads to form a
genome (also known as de novo sequence assembly) [1,4]; or on to a reference DNA
sequence, usually a genome, for downstream applications such as
single-nucleotide polymorphism (SNP) discovery [3], Chip-Seq [5] or RNA-Seq [6].
Here we focus on the latter type of alignments."
We focus on the latter.

% and in finding gene function
% [Def] genetic (relating to heredity or genes) vs. genomic (relating to the complete set of genes) 
% how are the 2 sequences compared?
% what is a sequence?
% where are the sequences coming from?
% how does the DB to store the sequences look like?
Smith-Waterman (SW)~\cite{sw} algorithm is one of the standard algorithms in
deciding how well two sequences align, i.e., how similar two sequences are.
% Compare target seq to search seq
However, alignment over a database of billions of sequences is a computationally
expensive task, and SW algorithm performs poorly. Alternative algorithms such as
BLAST~\cite{blast} or FASTA~\cite{fasta}, on the other hand, can run faster by trading
accuracy for performance. Contrary to SW, these algorithms are not guaranteed to
find the optimal local alignment.

- Growth rate estimations? Pure function of sequencing capabilities?

Three options:
- One to one: Pair-wise sequence alignment (PSA), e.g., SW
* One to many: A sequence is searched against a database of many sequences,
* e.g., BLAST 
- Many to many: Multiple sequence alignment (MSA)
Parallel variants of all algorithms exists.
[are these serving different purposes, or are these evolve as a function of
sequencing capabilities -- i.e., can each regarded be as a generalization of the
former?]

[Opens]

- Similarity metric not clear:
  
  Mutation and noisy machine reads matter in this context. We model these as
  abstracted out noise probabilities.

- The current implementation (at the high-level) pretty much looks like a BLAST
  variant

- Iso-alignment fidelity:

  BioCAM is always better.
}




==> overviewfig1.tex <==
\begin{figure*}[htp]
%\vshrink{0.7}
\begin{center}
\begin{minipage}{.3\textwidth}
  \includegraphics[width=\columnwidth]{FIG/micro_filterU.pdf}
\vshrink{0.4}
  \caption{Filter Unit (FilterU)
  \label{fig:fu}}
\end{minipage}
\hspace{1cm}
\begin{minipage}{.49\textwidth}
  \subfloat[{\em full match}]{  
	\includegraphics[width=0.42\textwidth]{FIG/fullmatch.pdf}
		\label{fig:fullmatch}
 } 
  \subfloat[{\em fragmented match}]{  
	\includegraphics[width=0.42\textwidth]{FIG/rightpartialmatch.pdf}
		\label{fig:partmatchright}
  }
  \caption{Full (a) and fragmented (b) match in the array.
  \label{fig:match}}
\end{minipage}
\end{center}
\vshrink{0.7}
\end{figure*}



==> relMicro.tex <==
\noindent Smith-Waterman (SW)~\cite{sw} algorithm is one of the standard algorithms in
deciding how well two sequences align, i.e., how similar two sequences are.
% Compare target seq to search seq
However, alignment over a database of billions of sequences is a computationally
expensive task where the SW algorithm performs poorly. Alternative algorithms
such as BLAST~\cite{blast} or FASTA~\cite{fasta}, on the other hand, can run
faster by trading
%accuracy
alignment fidelity for performance. Contrary to SW, these algorithms are not
guaranteed to find the optimal local alignment.



==> scalfigs.tex <==
\begin{figure}[h]
%\vshrink{0.7}
\begin{center}
%\hspace{-0.1cm}
  \includegraphics[width=0.9\columnwidth]{FIG/postmicro17_inps_combined.pdf} 
  \caption{
	%Throughput gain of 
	Throughput scalability of BioCAM vs. Barracuda.
	%for different query sizes.
  \label{fig:inps}}
\end{center}
\vshrink{0.6}
\end{figure}



==> shortIndel.tex <==
\noindent{\redHL {\bf Mutation-induced short indels:}}



==> similarMicro.tex <==
\noindent 
Fig.~\ref{fig:tcamCell} depicts a representative resistive TCAM cell.  The two
resistors attached to the access transistors $Acc_1$ and $Acc_2$, respectively, 
carry the data bit value
$D$ and its complement $\overline{D}$. 
%connected to the {\em Search Line} ($SL$) and its complement
%$\overline{SL}$ over the access transistors $Acc_1$ and $Acc_2$, respectively, carry the data bit value
%$D$ and its complement $\overline{D}$.  
The high (low) resistance value $R_{high}$ ($R_{low}$) encodes logic 1 (0).
The third resistor 
%connected
%to the {\em Search X Line} ($SXL$) over 
attached to $Acc_3$
%, on the other
%hand, 
is hardwired to logic 1, hence its resistance remains constant at $R_{high}$. 
%

\begin{figure}[h]
\vshrink{0.2}
  \begin{center}
%\hspace{-0.62cm}
  \includegraphics[width=0.4\textwidth]{FIG/tcamCell.pdf}
\vshrink{0.1}
  \caption{Resistive TCAM cell~\cite{ipekTCAM}.
  \label{fig:tcamCell}}
\end{center}
\vshrink{0.5}
\end{figure}

To search for logic 0, {\em Search Line} ($SL$) is set to 0, and its complement
$\overline{SL}$ to 1, such that $Acc_2$ turns on; $Acc_1$ off.  Thereby only the
resistor carrying $\overline{D}$, $R$, gets connected to the {\em Match Line}
($ML$).
%
If the cell content was 0, i.e., ${D}=0$ and $\overline{D}=1$, there would be a match,
and $R=R_{high}$ applies.  
Otherwise, if the cell content was 1, i.e., ${D}=1$ and $\overline{D}=0$, there
would be a mismatch, and $R=R_{low}$ applies. 
A symmetric discussion holds for searching for logic 1. 
%
On a per TCAM cell basis, $R_{high}$ connected to $ML$ indicates a match,
$R_{low}$, a mismatch.
%
To search for X, both $SL$ and
$\overline{SL}$ are set to 0, and {\em Search X Line} 
%($SXL$) 
to 1,  such that
only the hard-wired $R_{high}$ attached to $Acc_3$ is connected to $ML$. 
%As this resistor is hardwired to $R_{high}$, 
This is why search for X always renders a match, independent of the value of $D$.

%To summarize, on a per TCAM cell basis, $R_{high}$ connected to $ML$ indicates a match,
%$R_{low}$, a mismatch. 
Each cell within each row contributes to the effective resistance connected to
$ML$, $R_{eff}$,  by  $R_{high}$ ($R_{low}$) on a match (mismatch).
%a specific resistance value which reflects the
%(mis)match outcome within the cell. 
The {\em Sense Amplifier} SA (connected to the $ML$) in each row signals a
(mis)match for the entire row depending on the value of $R_{eff}$.  
%In a TCAM array based on the cell from Fig.~\ref{fig:tcamCell}, unless
%all bits within a row match, SA would always signal a mismatch for the entire row.
%For
%instance, in an array with a row size of 1Kbits,  
SA would only signal a match,
if all cells match, i.e., 
if each cell contributes to $R_{eff}$  by $R_{high}$. Let us call
the $R_{eff}$ in this case $R_{match}$.
SA would signal a mismatch if at least one cell mismatches, i.e.,
contributes to $R_{eff}$ by $R_{low}$. The value of $R_{eff}$ in this case 
evolves with the number of mismatches, and 
%$R_{eff}$ 
assumes the closest value to
$R_{match}$ under a single-cell (bit) mismatch. 
%Let us call this $R_{eff}$ $R_{mismatch}$.  

In a TCAM array based on the cell from Fig.~\ref{fig:tcamCell}, unless
all bits within a row match, SA would always signal a mismatch for the entire row.
However, due to NGS platform induced noise and mutations (as detailed in
Section~\ref{sec:pr}) a matching {\em query} may indeed have a few bases
different from the corresponding sub-sequence of the {\em reference}.
%according to the data representation adopted by \arch, as explained in
%Section~\ref{sec:encode}, each single-base mismatch 
%in the \ssq\ and the \srg\
%strings 
%would generate a 2-bit mismatch in the TCAM array.
To resolve this discrepancy, 
\arch\ deploys tunable SAs which associate a wider
$R_{eff}$ range with a row-wide match. 
%
These SAs can be tuned to signal a row-wide match when
less than a given 
%{\em threshold} ({\em t}) 
number {\em t} of bits mismatch, which translates into
less than {\em t} $R_{low}$s
connected to $ML$. We will refer to 
%this number 
{\em t} as {\em tolerance}, which
represents an adjustable design
parameter. 

The gap between $R_{eff}$ levels corresponding to different number of mismatching bits
decreases as the number of mismatching bits grows, complicating SA design. 
At the same time,
due to PVT (Process, Voltage, Temperature) variations, 
%and other sources of noise,
individual TCAM cell resistance levels may notably deviate from nominal $R_{high}$ or $R_{low}$,
leading to divergence of such $R_{eff}$ levels from their expected values.
Section~\ref{sec:sensest} details \arch's variation-aware SA design.
%and quantifies
%its false positive rate (i.e., the rate at which the SA signals a match where
%the number of mismatches remains higher than  {\em tolerance}). 
%{This design cannot result in false negatives by construction.} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\ignore{
Section~\ref{sec:eval}
quantifies sensing inaccuracies for different similarity thresholds and array sizes.
}

\ignore{
Hence, adjusting the sensing mechanism becomes more challenging as we try
to move the accepted threshold to lower $R_{eff}$ regions.
For instance, let us assume that up to a 3-base difference is acceptable to
signal a match. 
This means a $R_{eff}$ featuring 9 $R_{low}$s would lead to a match; 12 and more
$R_{low}$s, to a mismatch. Variation may render the $R_{eff}$ in the first case
lower than the latter, which would lead to a failure in sensing.

Since similarity is a fuzzy concept unlike exact match, such inaccurarcies (if not negligible)
can be tolerated by definition. Specefically in sequence alignment applications,
a single strict expected similarity threshold does not exist. So, fualts of sensing
similarity (if small) can be tolerated by these applications. 
These inaccuracies can cause negligible levels of uncertainty, rather than
leading to produce unacceptable or wrong results.
}

\ignore{
On a match (mismatch), each cell contributes to $ML$ by
$R_{high}$ ($R_{low}$). For instance, in an array with row
size of 1Kbits, on a match, 1K $R_{high}$s get connected
to $ML$. Conventional SAs associate only this case with a match. 
However, if only 90\% of the cells are matching the
query, 90\%$\times$1K $R_{high}$s and 10\%$\times$1K $R_{low}$s get connected to
$ML$. This would lead to a different effective resistance $R_{eff}$, lower
in comparison to the former case. 
$R_{eff}$ decreases with the number of mismatches per cell. Conventional SAs would not
associate any such $R_{eff}$ with a match. 
Tunable SAs in the TCAM arrays of \arch, on the other hand, can associate such $R_{eff}$
as a match. 
For instance, these SAs can be tuned to trigger a match signal when
less than 5 bits are mis-matching, which translates into less than 5 $R_low$s
connected to ML. The SA matching threshold is tunable.
The gap between $R_{eff}$ levels corresponding to different number of mismatching bits
decreases as the number of mismatching bits grows. 
Besides, 
}

\ignore{
We know that different genomes are not exactly the same,
although they are %more than 99\% 
similar. 
%Differences between two genomes come from polymorphism rate 
%(the natural differences in genomes) and the errors in measurements
%[XXX lecture]. 
Hence, in designing an alignment accelerator, 
we are looking for Similarity between a sub-sequence
and the reference genome, rather than an exact match. Currently in TCAM arrays, 
sense amplifiers are designed to detect the exact match. 
So, even a single bit mismatch leads to
triggering a mismatch signal for that row. We need to change
the 
%design of sense amplifier 
sensing mechanism in a way that {\em similarity} can be captured, as well as a {\em match}.

First, we take a look at how match detection is performed
in TCAMs. On a match (mismatch), each cell connects
an $R_{high}$ ($R_{low}$) to the Match Line (ML). For instance, in an array with row
size of 100 bits, on an exact match, 100 $R_{high}$s are connected
to the ML. However, if 90\% of the cells are matching the
query, 90 $R_{high}$s and 10 $R_{low}$s are connected to the
ML. This will lead to a different effective resistance, lower
in comparison to the exact match case. Since TCAMs are
designed to find exact matches, sense amplifiers are tuned to
%should be
%accurate enough to 
sense the difference between an exact
match and a case that only a single bit mismatches, which
means only a single $R_{low}$ is connected to the ML. 

To capture similarity rather than match-only, sense amplifier 
should be adjusted accordingly to accept a lower effective resistance
as a match. For instance, it can be set to triger a match signal when
less than 5 bits are mis-matching, which means having less than 5 $R_low$s
connected to the ML. This way, be changing the matching threshold of sense
amplifiers, TCAM arrays are capable of capturing similarity when difference
is small enough.

[[{\bf we may include UCSD comparison here}]]

As shown in Figure [XXX resistance gaps, like what shown in oral defense and Engin's],
the gap between effective resistance levels under different number of mismatching bits
decreases as number of mismatching bits grows. 
Besides, due to process variation and other sources of noise,
TCAM cells' resistance deviates from being exaxctly $R_{high}$ or $R_{low}$.
Hence, adjusting the sensing mechanism becomes more challenging as we try
to move the accepted threshold to lower effective resistance regions.
For instance let us assume that up to 3 bp difference is acceptable.
This means 6 $R_{low}$s are considered as a match, while having 8 and more $R_{low}$s
connected to the ML is not a match anymore. Then, due to process variation, there
might be scenarios that resistance levels of a row containing 6 $R_{low}$s become
less than a row with 8 ${R_{high}}$s, which will lead to a failure in sensing.

Since similarity is a fuzzy concept unlike exact-match, such inaccurarcies (if not negligible)
can be tolerated by definition. Specefically in sequence alignment applications,
a single strict expected similarity threshold does not exist. So, fualts of sensing
similarity (if small) can be tolerated by these applications. 
These inaccuracies can cause negligible levels of uncertainty, rather than
leading to produce unacceptable or wrong results.
In Section XXX, we
quantify these sensing inaccuracies for different similarity thresholds and array sizes.

 

[[XXX we may want to eliminate rest of this section]]

This is
why small $\frac{R_{high}}{R_{low}}$ ratio makes the design of sense 
amplifier much more challenging (XXX cite Engin). Besides, as the size of 
array and consequently the rows increase, sensing margin 
becomes smaller, leading to more challenging sense amplifier
design. Moreover, the other challenge in designing a sense
amplifier is that $R_{high}$ and $R_{low}$ are prone to process 
variation. So, the final effective resistance connected to the sense
line, $R_{eff}$, varies from the expected value. As shown in [cite
Hassan UCI], process variation alone can lead to scenarios
that sense amplifier fails to detect a match or a mismatch.
This variation should be considered in designing the sense
amplifier too.

Similarity is a fuzzy concept by definition, rather than a
simple match or mismatch. Acceptability of a similarity
level between two sequences depends on the application. In
genome alignment problem, we are looking for similar 
sequences, rather than exactly identical ones. So, sense 
amplifier can tolerate noise. In other words, considering process
variation and other limits, we can design a sense amplifier
that captures a match when we have more than a specific
number of bits (let say 90 bits) matching the query;
however, due to the effect of noise, sense amplifier may 
trigger a match signal on lower number of matching bits (like
80) as well. This fuzziness is acceptable, as long as we make
sure that all sequences with more than a specific number of
bits matching will trigger a match signal. We call this safe
threshold $R_{match}$, and we report it in percents. For instance,
a sense amplifier designed for $R_{match}$ = 75\% and row size of
128 bits, triggers match signal always when more than 96
bits are matching the query, while sometimes it may trigger
a false match signal when we have less than 96 bits matching. 
So, it can trigger false positives, but false negatives are
not acceptable. False positives are not catastrophic failures.
They are rather less similar matches. 
%We show in SectionXXX how
%many False Positives are generated and how different they are.
In section XXX, for different array sizes and
PVT conditions, we quantify the rate of false positives and
consequently, the acceptability of sense amplifier for this application. 
Besides, we show how different the false positives can get from the
expected threshold.

[[XXX we may want to eliminate this pragraph completely]]
Similarity rate between a sub-sequence and the reference
genome is always low, except where it aligns, which is very
rare. In alignment applications, we are looking for more than
95\% of the bps matching the reference. We use this  
in designing the sense amplifier to decrease the number of
false positives. Basically, we set the goal of designing the
sense amplifier to capture all the cases with similarity above
$R_{match}$. At the same time, we try to decrease the probability 
of generating a false positive for cases with low similarity. 
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


